Almost all optimally coloured complete graphs contain a rainbow Hamilton path

A subgraph $H$ of an edge-coloured graph is called rainbow if all of the edges of $H$ have different colours. In 1989, Andersen conjectured that every proper edge-colouring of $K_{n}$ admits a rainbow path of length $n-2$. We show that almost all optimal edge-colourings of $K_{n}$ admit both (i) a rainbow Hamilton path and (ii) a rainbow cycle using all of the colours. This result demonstrates that Andersen's Conjecture holds for almost all optimal edge-colourings of $K_{n}$ and answers a recent question of Ferber, Jain, and Sudakov. Our result also has applications to the existence of transversals in random symmetric Latin squares.

==> figs/assymetrical-mini-absorber.tex <==
\begin{figure}
  \centering
    \begin{tikzpicture}%[scale = 2]
    \tikzstyle{vtx}=[draw, fill, circle, scale = .5];
    \tikzstyle{link}=[snake=zigzag];
    % \node[label=-45:{\huge $v$}] (v) at ($(2)!.66!(5)$) {}


    \node[label=left:{\Large $v_1$}, vtx] (v) at (0, 0) {};

    \node[vtx] (t1) at ($(v) + (30:1)$) {};
    \node[vtx] (b1) at ($(v) + (-30:1)$) {};

    \node[vtx] (t2) at ($(t1) + (1, 0)$) {};
    \node[vtx] (b2) at ($(b1) + (1, 0)$) {};

    \node[vtx] (t3) at ($(t2) + (1, 0)$) {};
    \node[vtx] (b3) at ($(b2) + (1, 0)$) {};

    \draw (v) -- (t1);% node[midway] {\Large 1};
    \draw (t1) -- (b1);% node[midway] {\Large 3};
    \draw (b1)-- (v);% node[midway] {\Large 2};

    \draw (t2) -- (b2);% node[midway] {\Large 3};
    \draw (t2) -- (t3);% node[midway] {\Large 1};
    \draw (b2) -- (b3);% node[midway] {\Large 2};
    \draw (t3) -- (b3) node[midway] {\Large $c_1$};

    \draw[link] (t1) -- (b2);
    \draw[link] (t2) -- (b3);

    \node[vtx] (t'1) at ($(t3) + (1, 0)$) {};
    \node[vtx] (b'1) at ($(b3) + (1, 0)$) {};

    \node[vtx] (t'2) at ($(t'1) + (1, 0)$) {};
    \node[vtx] (b'2) at ($(b'1) + (1, 0)$) {};

    \node[vtx] (t'3) at ($(t'2) + (1, 0)$) {};
    \node[vtx] (b'3) at ($(b'2) + (1, 0)$) {};

    \draw (v) .. controls ($(v) + (0, 1)$) and ($(t'1) + (0, .5)$) .. (t'1);% node[midway] {\Large 1};
    \draw  (v) .. controls ($(v) + (0, -1)$) and ($(b'1) + (0, -.5)$) .. (b'1);% node[midway] {\Large 2};
    \draw (t'1) -- (b'1);% node[midway] {\Large 3};


    \draw (t'2) -- (b'2);% node[midway] {\Large 3};
    \draw (t'2) -- (t'3);% node[midway] {\Large 1};
    \draw (b'2) -- (b'3);% node[midway] {\Large 2};
    \draw (t'3) -- (b'3) node[midway] {\Large $c_2$};

    \draw[link] (t'1) -- (b'2);
    \draw[link] (t'2) -- (b'3);

        \draw[link] (t3) -- (b'1);
    %\draw[decorate, decoration=zigzag] (t'1) .. controls ($(t'1) + (0, .5)$) and ($(t3) + (0, .5)$) .. (t3);


    \node[label=left:{\Large $v_2$}, vtx] (bv) at (0, -2.5) {};

    \node[vtx] (bt1) at ($(bv) + (30:1)$) {};
    \node[vtx] (bb1) at ($(bv) + (-30:1)$) {};

    \node[vtx] (bt2) at ($(bt1) + (1, 0)$) {};
    \node[vtx] (bb2) at ($(bb1) + (1, 0)$) {};

    \node[vtx] (bt3) at ($(bt2) + (1, 0)$) {};
    \node[vtx] (bb3) at ($(bb2) + (1, 0)$) {};

    \draw (bv) -- (bt1);% node[midway] {\Large 1};
    \draw (bt1) -- (bb1);% node[midway] {\Large 3};
    \draw (bb1)-- (bv);% node[midway] {\Large 2};

    \draw (bt2) -- (bb2);% node[midway] {\Large 3};
    \draw (bt2) -- (bt3);% node[midway] {\Large 1};
    \draw (bb2) -- (bb3);% node[midway] {\Large 2};
    \draw (bt3) -- (bb3) node[midway] {\Large $c_1$};

    \draw[link] (bt1) -- (bb2);
    \draw[link] (bt2) -- (bb3);

    \node[vtx] (bt'1) at ($(bt3) + (1, 0)$) {};
    \node[vtx] (bb'1) at ($(bb3) + (1, 0)$) {};

    \node[vtx] (bt'2) at ($(bt'1) + (1, 0)$) {};
    \node[vtx] (bb'2) at ($(bb'1) + (1, 0)$) {};

    \node[vtx] (bt'3) at ($(bt'2) + (1, 0)$) {};
    \node[vtx] (bb'3) at ($(bb'2) + (1, 0)$) {};

    \draw (bv) .. controls ($(bv) + (0, 1)$) and ($(bt'1) + (0, .5)$) .. (bt'1);% node[midway] {\Large 1};
    \draw (bv) .. controls ($(bv) + (0, -1)$) and ($(bb'1) + (0, -.5)$) .. (bb'1);% node[midway] {\Large 2};
    \draw (bt'1) -- (bb'1);% node[midway] {\Large 3};


    \draw (bt'2) -- (bb'2);% node[midway] {\Large 3};
    \draw (bt'2) -- (bt'3);% node[midway] {\Large 1};
    \draw (bb'2) -- (bb'3);% node[midway] {\Large 2};
    \draw (bt'3) -- (bb'3) node[midway] {\Large $c_2$};

    \draw[link] (bt'1) -- (bb'2);
    \draw[link] (bt'2) -- (bb'3);

    \draw[link] (bt3) -- (bb'1);
    \draw[decorate, decoration=zigzag] (b1) .. controls ($(b1) + (0, -.5)$) and ($(bt'3) + (0, .5)$) .. (bt'3);

  \end{tikzpicture}%}
    \caption{
    An absorber $(\mathcal A, \mathcal P, T, H)$, where $\mathcal P$ links $\cup_{i=1}^3 M_i$ and $T = M\cup \bigcup_{P\in\mathcal T} P$, where $\mathcal T$ links $M_4$. %such that $\bigcup_{A\in\mathcal A} A \cup \bigcup_{P\in\mathcal P} P \cup T$ is contained in $(V', C', G')$ with $\gamma$-bounded remainder.
  }
  \label{fig:building-absorber}
\end{figure}
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../andersen"
%%% End:

